RACE-OC Project: Rotation and variability in the open cluster NGC2099 (M37)

Rotation and solar-type magnetic activity are closely related to each other in stars of G or later spectral types. Presence and level of magnetic activity depend on star's rotation and rotation itself is strongly influenced by strength and topology of the magnetic fields. Open clusters represent especially useful targets to investigate the connection between rotation and activity. The open cluster NGC2099 has been studied as a part of the RACE-OC project, which is aimed at exploring the evolution of rotation and magnetic activity in the late-type members of open clusters of different ages. Time series CCD photometric observations of this cluster were collected during January 2004. The relations between activity manifestations, such as the light curve amplitude, and global stellar parameters are investigated. We have discovered 135 periodic variables, 122 of which are candidate cluster members. Determination of rotation periods of G- and K-type stars has allowed us to better explore evolution of angular momentum at an age of about 500 Myr. A comparison with the older Hyades cluster (~625 Myr) shows that the newly determined distribution of rotation periods is consistent with the scenario of rotational braking of main-sequence spotted stars as they age. However, a comparison with the younger M34 cluster (~200 Myr) shows that the G8-K5 members of these clusters have the same rotation period distribution, that is G8-K5 members in NGC2099 seem to have experienced no significant braking in the age range from ~200 to ~500 Myr. Finally, NGC2099 members have a level of photospheric magnetic activity, as measured by light curve amplitude, smaller than in younger stars of same mass and rotation, suggesting that the activity level also depends on some other age-dependent parameters.

==> graphicx.tex <==
% Plain TeX interface to graphicx package.
% David Carlisle


\input miniltx

\def\Gin@driver{dvips.def}
\input graphicx.sty


\resetatcatcode



